Rapid Exploration for Open-World Navigation with Latent Goal Models

We describe a robotic learning system for autonomous exploration and navigation in diverse, open-world environments. At the core of our method is a learned latent variable model of distances and actions, along with a non-parametric topological memory of images. We use an information bottleneck to regularize the learned policy, giving us (i) a compact visual representation of goals, (ii) improved generalization capabilities, and (iii) a mechanism for sampling feasible goals for exploration. Trained on a large offline dataset of prior experience, the model acquires a representation of visual goals that is robust to task-irrelevant distractors. We demonstrate our method on a mobile ground robot in open-world exploration scenarios. Given an image of a goal that is up to 80 meters away, our method leverages its representation to explore and discover the goal in under 20 minutes, even amidst previously-unseen obstacles and weather conditions. Please check out the project website for videos of our experiments and information about the real-world dataset used at https://sites.google.com/view/recon-robot.

==> figures/bottleneck_graph.tex <==

\newcommand{\shadowcolor}[0]{black!20}
\newcommand{\encodercolor}[0]{Magenta!100}
\newcommand{\decodercolor}[0]{NavyBlue!100}

\newcommand{\bottleneckgraph}[0]{
\node [matrix,matrix anchor=mid, column sep=25pt, row sep=40pt, ampersand
replacement=\&,nodes={circle,thick,minimum size=1.5cm}] {
\& \node[draw=black] (Og)    {$O_g$}; \\
\& \node[draw=black] (Ztg)   {$Z_t^g$}; \\
\node[draw=black] (Ot) {$O_t$}; \& \&
\node[draw=black] (ADtg)   {$A_t^g,D_t^g$}; \\
};
\draw [->,\encodercolor,ultra thick] (Og) -- (Ztg) node[midway,rounded corners,fill=\shadowcolor] {\color{black}Encoder~{\color{\encodercolor}$p_\phi$}$(z_t^g|o_g,o_t)$}; 
\draw [->,\encodercolor,ultra thick] (Ot) -- (Ztg) ;
\draw [->,\decodercolor,ultra thick] (Ot) -- (ADtg);
\draw [->,\decodercolor,ultra thick] (Ztg) -- (ADtg) node[midway,rounded corners,fill=\shadowcolor] {\color{black}Decoder~{\color{\decodercolor}$q_\theta$}$(a_t^g, d_t^g|z_g^t,o_t)$};
}


==> figures/policy_arch.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp6326195379420629] 
\draw  [line width=3.75]  (79,186) .. controls (79,172.19) and (90.19,161) .. (104,161) .. controls (117.81,161) and (129,172.19) .. (129,186) .. controls (129,199.81) and (117.81,211) .. (104,211) .. controls (90.19,211) and (79,199.81) .. (79,186) -- cycle ;
%Shape: Circle [id:dp07150966584505625] 
\draw  [line width=3.75]  (79,64) .. controls (79,50.19) and (90.19,39) .. (104,39) .. controls (117.81,39) and (129,50.19) .. (129,64) .. controls (129,77.81) and (117.81,89) .. (104,89) .. controls (90.19,89) and (79,77.81) .. (79,64) -- cycle ;
%Shape: Circle [id:dp47466552593137235] 
\draw  [line width=3.75]  (260,186) .. controls (260,172.19) and (271.19,161) .. (285,161) .. controls (298.81,161) and (310,172.19) .. (310,186) .. controls (310,199.81) and (298.81,211) .. (285,211) .. controls (271.19,211) and (260,199.81) .. (260,186) -- cycle ;
%Shape: Circle [id:dp8060843510267749] 
\draw  [line width=3.75]  (435,90) .. controls (435,76.19) and (446.19,65) .. (460,65) .. controls (473.81,65) and (485,76.19) .. (485,90) .. controls (485,103.81) and (473.81,115) .. (460,115) .. controls (446.19,115) and (435,103.81) .. (435,90) -- cycle ;
%Shape: Circle [id:dp6080491951441201] 
\draw  [line width=3.75]  (435,158) .. controls (435,144.19) and (446.19,133) .. (460,133) .. controls (473.81,133) and (485,144.19) .. (485,158) .. controls (485,171.81) and (473.81,183) .. (460,183) .. controls (446.19,183) and (435,171.81) .. (435,158) -- cycle ;
%Rounded Rect [id:dp06925011321182661] 
\draw  [line width=1.5]  (423,85) .. controls (423,64.57) and (439.57,48) .. (460,48) -- (460,48) .. controls (480.43,48) and (497,64.57) .. (497,85) -- (497,163) .. controls (497,183.43) and (480.43,200) .. (460,200) -- (460,200) .. controls (439.57,200) and (423,183.43) .. (423,163) -- cycle ;
%Straight Lines [id:da24005799374958503] 
\draw [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][line width=1.5]    (139,186) -- (248,186) ;
\draw [shift={(251,186)}, rotate = 180] [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][line width=1.5]    (17.05,-5.13) .. controls (10.84,-2.18) and (5.16,-0.47) .. (0,0) .. controls (5.16,0.47) and (10.84,2.18) .. (17.05,5.13)   ;
%Straight Lines [id:da15717536532534437] 
\draw [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][line width=1.5]    (134,80) -- (252.55,164.26) ;
\draw [shift={(255,166)}, rotate = 215.4] [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][line width=1.5]    (17.05,-5.13) .. controls (10.84,-2.18) and (5.16,-0.47) .. (0,0) .. controls (5.16,0.47) and (10.84,2.18) .. (17.05,5.13)   ;
%Straight Lines [id:da35606642228007757] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (319,185) -- (413.28,141.26) ;
\draw [shift={(416,140)}, rotate = 515.11] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (17.05,-5.13) .. controls (10.84,-2.18) and (5.16,-0.47) .. (0,0) .. controls (5.16,0.47) and (10.84,2.18) .. (17.05,5.13)   ;
%Straight Lines [id:da9302275172497433] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (139,68) -- (412.05,116.48) ;
\draw [shift={(415,117)}, rotate = 190.07] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (17.05,-5.13) .. controls (10.84,-2.18) and (5.16,-0.47) .. (0,0) .. controls (5.16,0.47) and (10.84,2.18) .. (17.05,5.13)   ;

% Text Node
\draw (783,203) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1.44em}{1.73em}\selectfont] [align=left] {z};
% Text Node
\draw (162,205) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 189; green, 16; blue, 224 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{42.404375pt}\setlength\topsep{0pt}
\begin{center}
\textbf{encoder}\\
\end{center}

\end{minipage}};
% Text Node
\draw (314,45) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 189; green, 16; blue, 224 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{42.404375pt}\setlength\topsep{0pt}
\begin{center}
\textbf{\textcolor[rgb]{0.96,0.65,0.14}{decoder}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (95,55) node [anchor=north west][inner sep=0.75pt]    {$O_{t}$};
% Text Node
\draw (93,177) node [anchor=north west][inner sep=0.75pt]    {$O_{g}$};
% Text Node
\draw (180,222) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,opacity=1 ]  {$p_{\phi }$};
% Text Node
\draw (334,60) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ]  {$q_{\theta }$};
% Text Node
\draw (275,174) node [anchor=north west][inner sep=0.75pt]    {$Z^{g}_{t}$};
% Text Node
\draw (450,78) node [anchor=north west][inner sep=0.75pt]    {$A^{g}_{t}$};
% Text Node
\draw (450,147) node [anchor=north west][inner sep=0.75pt]    {$D^{g}_{t}$};


\end{tikzpicture}


